Buoyancy driven motion of non-coalescing inertial drops: microstructure modeling with nearest particle statistics

In this study, we analyze the various arrangements that droplets can form within dispersed buoyant emulsions, which we refer to as the study of microstructure. To this end, we have developed a novel algorithm that effectively prevents numerical coalescence between drops while maintaining a reasonable computational cost. This algorithm is integrated into the Volume of Fluid (VoF) method and implemented using the open-source code http://basilisk.fr. Subsequently, we perform Direct Numerical Simulations (DNS) of statistically steady state mono-disperse buoyant emulsion over a broad range of dimensionless parameters, including the particle volume fraction ($\phi$), the Galileo number ($Ga$) and the viscosity ratio ($\lambda$). We make use of nearest particle statistics to quantify the microstructure properties. As predicted by Zhang et al. (2023), it is demonstrated that the second moment of the nearest particle pair distribution can effectively quantify microstructural features such as particle clusters and layers. Specifically, the findings are: (1) In moderately inertial flows ($Ga = 10$), droplets form isotropic clusters. In high inertial regimes ($Ga = 100$), non-isotropic clusters, such as horizontal layers, are more likely to form. (3) The viscosity ratio plays a significant role in determining the microstructure, with droplets that are less viscous or equally viscous as the surrounding fluid tending to form layers preferentially. Overall, our study provides a quantitative measure of the microstructure in terms of $Ga$, $\phi$ and $\lambda$.

==> microstructure/Time_of_interaction.tex <==
As the previous section focused solely on the geometry of the microstructure, we now provide a more comprehensive view of the timescale that drives the interaction between nearest pairs, as well as the times scale involved for the tensor $\textbf{R}(\textbf{x},t)$.

\subsubsection*{A transport equation for the microstructure geometry}
We have seen in the previous section that the tensor $\textbf{R}(\textbf{x},t)$ is able to describe the geometry of the microstructure. 
To determine how this microstructure evolves in time we make use of the transport equation of $P_\text{nst}(\textbf{x},\textbf{r},t,a)$ derived in \citet{zhang2023evolution}.
As it is a rather new formalism we recall this equation here, 
\begin{equation}
    \pddt P_\text{nst}
    + \pdda P_\text{nst}
    + \pddx \cdot  (\textbf{u}^\text{nst}_p P_\text{nst})
    + \pddr \cdot  (\textbf{w}^\text{nst}_p P_\text{nst})
    = \delta(a)P(\textbf{x},\textbf{r},0,t)
    - \frac{P_\text{nst}}{\tau^\text{nst}(\textbf{x},\textbf{r},t,a)}
    \label{eq:dt_Pnst}
\end{equation}
where $\textbf{u}^\text{nst}_p$ and $\textbf{w}_{p}^\text{nst}$ are the conditioned average of the particle phase velocity and relative velocity, respectively, defined \ref{sec:methodo}. 
The left-hand side of \ref{eq:dt_Pnst} corresponds to the convective derivative of $P_\text{nst}$ with respect to the nearest particle statistics' phase space. 
The first term on the right-hand side of \ref{eq:dt_Pnst} account for the creation of the nearest pairs, thus it is non-zero only for the age $a = 0$, as witnessed by the Dirac delta function $\delta(a)$. 
The second term on the right-hand side is the contribution from the destruction of the nearest pairs.
Where we defined $1/\tau^\text{nst}(\textbf{x},\textbf{r},t,a)$ as the rate of destruction of pairs of particles of age $a$ with relative position $\textbf{r}$.
Additionally, we define the mean rate of destruction, $1/\tau_p$, by, 
\begin{equation*}
    \frac{n_p}{\tau_p}(\textbf{x},t) = 
    \int_{0}^\infty
    \int_{\mathbb{R}^3}
    \frac{P_\text{nst} }{\tau^\text{nst}}(\textbf{x},\textbf{r},t,a)
    da d\textbf{r}. 
\end{equation*}
As we show now, $\tau_p$ is of great importance as it governs the timescale of the microstructure.

By taking the partial time derivative of \ref{eq:R}, and utilizing \ref{eq:dt_Pnst}, we obtain an equation for $\textbf{R}(\textbf{x},t)$, it reads,
\begin{equation*}
    \pddt (n_p\textbf{R})
    + \pddx \cdot [n_p(\textbf{u}_p\textbf{R}
    + \textbf{R}^\text{Re})]
    = 
    - \frac{n_p\textbf{R}}{\tau_p}
    +n_p\textbf{B}
    + n_p\textbf{D}
    + n_p\textbf{W}
    \label{eq:dt_R}
\end{equation*}
With,
\begin{align*}
    n_p \textbf{R}^\text{Re}(\textbf{x},t)
    =
    \int_{0}^\infty
    \int_{\mathbb{R}^3}
    \textbf{rr}(\textbf{u}^\text{nst}_p - \textbf{u}_p)
    P(\textbf{x},\textbf{r},t,a)
    d\textbf{r}da,\\
    n_p \textbf{B}(\textbf{x},t)
    =
    \int_{0}^\infty
    \int_{\mathbb{R}^3}
    \textbf{rr}
    P(\textbf{x},\textbf{r},t,0)\delta(a)
    d\textbf{r}da, \\
    n_p\textbf{D}(\textbf{x},t) = 
    \int_{0}^\infty
    \int_{\mathbb{R}^3} \textbf{rr}
    \left[
        \frac{1}{\tau_p(\textbf{x},t)}
        - \frac{1}{\tau^\text{nst}(\textbf{x},\textbf{r},t,a)}
    \right]
    P_\text{nst}
    d\textbf{r}
    da,\\
    n_p \textbf{W}(\textbf{x},t) = 
    \int_{0}^\infty
    \int_{\mathbb{R}^3} \left[
        \textbf{r} \textbf{w}^\text{nst}_p
        + \textbf{w}^\text{nst}_p\textbf{r}
    \right]P_\text{nst}
    d\textbf{r}
    da.
\end{align*} 
The tensor $\textbf{R}^\text{Re}$ represent the flux due to velocity fluctuations. 
The source term $\textbf{B}$ is the averaged square relative position conditioned on the age $a=0$, meaning that it is related to the birth of the nearest particle pairs. 
In opposition to \textbf{D} which is related to the death of the particles pairs due to the presence of $\tau_p$ and $\tau_p^\text{nst}$.
Therefore, $\textbf{D}$ is the weighted average of $\textbf{rr}$ in terms of the destruction rate fluctuation fields. 
Likewise, $\textbf{B}$ is the weighted average of $\textbf{rr}$ on the Dirac distribution $\delta(a)$. 
The former term cancel out under the hypothesis that $1 / \tau^\text{nst}_p(\textbf{x},\textbf{r},t,a)$ is independent of age and relative position, in which case $\tau_p = \tau^\text{nst}_p$. 
Such simplification might be valid at high particle velocities fluctuation, however in our case we could not observe this independence with the DNS results.  
Additionally, the tenor $\textbf{W}(\textbf{x},t)$ is the correlation between the particles relative position and velocity.
Furthermore, due to the presence of the first term on the right-hand side of \ref{eq:dt_R}, we can state that $\textbf{R}(\textbf{x},t)$ will eventually relax within time, and that the relaxation time is $\tau_p$. 
In \citet{zhang2023evolution} they demonstrate that it is also the case for the particle-fluid-particle stress tensor.
In fact, this hold true for all nearest-neighbor averaged particles quantities, since this relaxation time is related to the transport equation of $P_\text{nst}(\textbf{x},\textbf{r},t,a)$, see \ref{eq:dt_Pnst}.
The main takeaway from \ref{eq:dt_R} is that, the microstructure as it is described by $\textbf{R}(\textbf{x},t)$, is motivated by 3 source terms, a term related to the weighted average of $\textbf{rr}$ on pair's birth and on pair's destruction, and a last one related to the particle relative velocity-position correlation. 


Since, $\textbf{R}(\textbf{x},t)$ follow a kinetic theory-like transport equation, it is interesting to discuss the possibility of implementing an equation such as \ref{eq:dt_R} in an Euler-Euler simulation framework. 
Attempting to close the source terms on the right-hand side of \ref{eq:dt_R} is very challenging. 
Instead, one could directly close $\textbf{R}(\textbf{x},t)$ based on the results of \ref{fig:A}, which are statistically steady state results of the microstructure. 
But then, how to know if the inertial effects related to the formation of the microstructure  (left hand-side of \ref{eq:dt_R}) are negligible ?
In fact, provided a relaxation time of the microstructure sufficiently small compared to the timescale of the flow, the derivatives in the right-hand side of \ref{eq:dt_R} might be negligible.
Therefore, $\textbf{R}(\textbf{x},t)$ can be expressed directly in terms of the flow parameters, provided that $\tau_p$ is smaller than the flow timescale. 
Then, the knowledge of $\textbf{R}(\textbf{x},t)$ by either solving \ref{eq:dt_R} or by obtaining direct closures laws, provides useful information for the closure terms in the Euler-Euler model.
For example, the averaged interphase momentum transfer is microstructure dependent. 
This, of course, requires having an expression for the closure terms in terms of the pair distribution function, which is not currently feasible.
Anyhow, the time $\tau_p$ is of major importance for two reasons: 
(1) it determines the timescale at which a statistically steady microstructure might be reached; 
(2) it provides useful information for the modeling of \ref{eq:dt_R}.

\subsubsection*{Mean age of interaction}

In this paragraph we evaluate the mean rate of destruction $1/\tau_p(\textbf{x},t)$. 
It is shown in a few paragraphs that the age distribution function is closely related to the mean rate of destruction. 
Therefore, let's first examine the age distribution, defined as, 
\begin{equation*}
    P_a(\textbf{x},t,a)
    = \frac{1}{n_p(\textbf{x},t)}
    \int_{\mathbb{R}^3}
    P_\text{nst}(\textbf{x},\textbf{r},t,a)
    d\textbf{r}.
\end{equation*} 
It is possible to derive an analytical formula for the age distribution, $P_a(\textbf{x},t,a)$, under the \textit{random destruction assumption} \citep{zhang2023evolution}.
This assumption state that the probability of particle pairs destruction, integrated on all position, is uncorrelated with the age of interaction.
In other worlds, we consider that any pairs of nearest neighbor can be broken apart equally likely regardless of the current age of the particle pair. 
Let us define $1/\tau_p^a(\textbf{x},t,a) = \frac{1}{n_p}\int_{\mathbb{R}^3}\tau^\text{nst} P_\text{nst}d\textbf{r}$, as the mean rate of pair destruction at age $a$, then this hypothesis state that $\tau^a_p$ is not a function of the age, such that $\tau^a_p(\textbf{x},t,a) = \tau_p(\textbf{x},t)$. 
It must be understood that $\tau^a_p$ is independent of the age, which does not imply that $\tau^\text{nst}_p$ is independent of the relative position, $\textbf{r}$, which is not true.
Under this assumption, which will be shown to be valid in our parameters' range, we can derive an analytical formula for the age distribution \citep{zhang2023evolution}, namely,
\begin{align}
    P_a(\textbf{x},t, a)  
    =\frac{e^{-a/\tau_p(\textbf{x},t)}}{\tau_p(\textbf{x},t)}.
    \label{eq:Pa}
\end{align} 
We can see that the age distribution is solely function of $\tau_p(\textbf{x},t)$ and that it is normalized to $1$.
Additionally, with this definition $\tau_p(\textbf{x},t)$, turns out to be equivalent to the first moment of the age distribution, such that, 
\begin{equation*}
    \int_{0}^\infty
    a P_\text{a}(\textbf{x},t,a)
    da
    =\tau_p(\textbf{x},t). 
\end{equation*}
Therefore, $\textbf{R}(\textbf{x},t)$ has a relaxation time equal to the first moment of the age distribution, which can be understood as the mean time of interaction of the particles pairs. 
In this sense it is intuitive to understand that the microstructure reach a statistically stable equilibrium after a time of the order of the mean particle interaction time. 

In \ref{fig:age_picture} (right) we display the dimensionless age distribution $P_a(\textbf{x},t,a)$ measured in our DNS, for different volume fraction, $\lambda =1$ and $Ga = 100$. 
The age is made dimensionless using the timescale, $U/d_p$ where $U$ is the averaged drift velocity.
The values of the Reynolds number based on the drift velocity are given in \ref{ap:age}, \ref{fig:Reall} for all our simulations. 
It is seen on \ref{fig:age_picture} (right) that the age distributions are rather well represented by the theoretical age distributions from \ref{eq:Pa}.
Consequently, the \textit{random destruction assumption} holds for these cases. 
\begin{figure}[h!]
    \centering
    \includegraphics[height = 0.3\textwidth]{image/HOMOGENEOUS_NEW/tau_Ga.pdf}
    \includegraphics[height = 0.3\textwidth]{image/HOMOGENEOUS_NEW/Dist/Pa_l_1_Ga_100.pdf}
    \caption{
    (left) Mean dimensionless age $\tau_a =  \int_0^\infty aP_a(\textbf{x},t,a)da$ in terms of the \textit{Galileo} number for different volume fraction :   
    ($\pmb\bigcirc$) $\phi = 0.01$; ($\pmb\triangle$) $ \phi = 0.05$; ($\pmb\square$) $\phi = 0.1$ ($\pmb\lozenge$) $\phi = 0.2$.
    The hollow symbols correspond to $\lambda = 1$, the filled symbols to $\lambda = 10$.
    (right) Age distribution function $P_a(\textbf{x},t,a)$ in terms of the dimensionless age, for $\lambda = 1$ and  $Ga = 100$.
    (dashed lines) Theoretical age distribution, see \ref{eq:Pa}. 
    Both the age and the mean age $\tau_a$ are made dimensionless with the drift velocity $U$ and the particle length scale $d_p$.  
    Black symbols represent the DNS results of \citet{zhang2023evolution} for hard sphere suspension with $\phi = 0.0168,0.0565,0.1341,0.2622$, corresponding to the symbols : $\pmb\times, \pmb +, \pmb\star , \pmb\triangledown$, respectively.
    }
    \label{fig:age_picture}
\end{figure}
In \ref{ap:age}  we provided the age distributions but for lower inertial effects, $Ga = 10$. 
It is seen that the age distribution at $\phi = 0.01$ and $Ga = 10$, exhibits a higher density for higher ages and is smaller for small ages, compared to the random distribution.
Therefore, at low \textit{Galileo} and low $\phi$ the \textit{random destruction assumption} doesn't seem to remain valid anymore. 
The \textit{random destruction assumption} must hold true for flows with high particle velocity fluctuation compared to the mean slip velocity, which induces randomness in particle interactions \citep{zhang2023evolution}. 
It is clear that for $\phi \rightarrow 0$, the particle phase fluctuation also tends to $0$, making this condition false. 
Apart from these two cases, it is reasonable to say that \ref{eq:Pa} is well representative of the age distribution function.

In \ref{fig:age_picture} (left) we displayed the dimensionless mean age for all our numerical experiment. 
Regarding the global trend of $\tau_p$, we can say that for almost all of our DNS, the time of interaction is higher for $\lambda = 1$ (hollow symbols) than for $\lambda = 10$ (filled symbols) at same $Ga$ and $\phi$.
Additionally,  $\tau_p$ seem to be well scaled by $U/d_p$ for $\phi  \leq 0.05$ as its values range between $2$ and $0.5$, which is reasonably close to $1$. 
However, $\tau_p$ is clearly superior for $\phi = 0.01$, and reaches a peak for $\phi=0.01$, $Ga=50$, $\lambda=1$.
This, may be correlated with the values of $A_{xx}$ on \ref{fig:A} which also reach a maximum for these parameters. 
Indeed, since $A_{xx}$ is rather high for these simulations, we know that particles are, on average, in a side-by-side configuration, which seems to be a stable configuration since $\tau_p$ is large too.
For $\lambda = 10$ we observe a smaller $\tau_p$ and a smaller $A_{xx}$ at $\phi = 0.01$ and $Ga = 50$, indicating that, on average, the interaction are not as long, while the microstructure is more isotropic. 
The dilute suspension of hard spheres, represented by a $\pmb\times$ symbol, seems to possess even lower $\tau_p$. 
This suggests that solid particles do not necessarily reach a stable equilibrium configuration in the dilute regime, unlike the bubble-like particles ($\lambda = 1$). 
This observation might be explained by the generation of more vorticity in the wake of viscous and solid particles, which makes the interactions less stable at these $Ga$ and $\phi$ values.
These pair interactions mechanisms have been investigated by \citet{yin2008lattice} when studying spherical bubbles and solid particles suspensions.
They reach the conclusion that the weaker wake generated by bubbles tends to make them spend more time in close horizontal orientations, in opposition to solid spherical particles. 
This finding strongly support the previous hypothesis. 
In summary, the mean age of interaction seem to be a good way to measure the particles pairs stability, since it provide a way to measure their interaction time. 
This time is shorter for increasing $\phi$, $\lambda$ and $Ga$, if $\phi \neq 0.01$ in which case it is non-monotonic with $Ga$. 

As mentioned above, $\tau_p(\textbf{x},t)$ is the relaxation time of $\textbf{R}(\textbf{x},t)$. 
Consequently, the microstructure relaxation of dilute suspensions is larger, especially at $Ga = 50$, and may need a consequent amount of time to reach a steady state regime. 
This implies that the terms on the left-hands side of \ref{eq:dt_R} may not be neglected and that direct closure for the microstructure in terms of $\phi$, $Ga$ and $\lambda$ may not be achievable at these large $\tau_p$. 
In turns, this relaxation time will be reflected on the drift velocity between both phases, which is microstructure dependent. 
\begin{figure}
    \centering
    \includegraphics[height=0.325\textwidth]{image/HOMOGENEOUS_NEW/CA/Relax2.pdf}
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/CA/Relax.pdf}
    \caption{
        (left) Average of the Reynolds number based on the instantaneous volume averaged drift velocity, $Re(t) = \rho_fU d /\mu_f$, with $U(t) = |\textbf{u}_p - \textbf{u}_f|$, divided by the mean Reynolds number $Re_m$ in terms of the dimensionless time. 
        (right) Running average of the Reynolds number $\widetilde{Re}(t)$ divided by the mean Reynolds number.
        For $\lambda = 1$ and $Ga = 50$ and two volumes fraction. 
        $\textbf{u}_p$ and $\textbf{u}_f$ are the particle and fluid phase volume averaged velocity at time $t$.
        The verticals gray lines indicate the values of $\tau_p$ all cases. 
        }
        \label{fig:relax}
\end{figure}
Indeed, in \ref{fig:relax} (right) we display the running average of the Reynolds number, based on the drift velocity, divided by the mean Reynolds number of the simulation for two values of $\phi = 0.01,0.1$ at $Ga = 50$ and $\lambda =1$. 
% It is seen that time, at which the simulation reaches a steady state regime is correlated with $\tau_p$. 
In this case we assume that two timescales are involved to bring the drift velocity to its statistically steady state regime. 
The first one is the particles' timescale, which is the time taken for a single particle to reach its own terminal velocity. 
The second timescale is the time taken for the microstructure to go from random, to its steady state microstructure. 
As a matter of fact, on \ref{fig:relax} we see that in the dilute regime ($\phi=0.01$) the rising velocity reaches its averaged value, at a time roughly equal to $100\sqrt{g/d}$ which is of the same order of magnitude than $\tau_p = 144\sqrt{g/d}$. 
On the contrary, when $\phi =0.1$ the averaged Reynolds number is indeed reached earlier ($t = 30\sqrt{g/d}$), despite the higher velocity fluctuations present in this case, see \ref{fig:relax} (left). 
The particle timescale is the same for both cases displayed \ref{fig:relax}, since only the volume fraction changes.
Additionally, the Statistical samples are supposed to be equivalent at same time since each  case posses the same number of droplets per domain. 
Thus, the changes in relaxation time is solely due to the microstructure relaxation timescale. 
Therefore, in support of the theory, $\tau_p$ seems capable of predicting the relaxation time of the microstructure.


The rising velocity of particles is directly correlated to the interphase drag force in sedimentation problems \citep{jackson1997locally}. 
Therefore, in the objective of finding closure terms for the averaged models, one must perform DNS for a time longer than $\tau_p$ plus the particle timescale, to allow the microstructure to relax adequately.
Then by performing an ensemble average procedure, one is able to build drag force models. 
Once established, these models will remain valid only under the condition where the timescale of the macroscopic flow significantly exceeds $\tau_p(\textbf{x},t)$ plus the particle timescale.
Indeed, these models have been built for relaxed microstructure and can be utilized only in this context.
Consequently, $\tau_p$ among other factors such as the particle relaxation time, provides a threshold value for the timescale not achievable in Euler-Euler models. 

\subsubsection*{Particle pairs approach velocity}

\tb{je ne suis plus tellement sur de la pertinience de cette section}

In the next section we will be interested in the velocity fields $\textbf{w}_p^\text{nst}$ since it appear in the source term $\textbf{W}(\textbf{x},t)$, which is at the origin of the modifications of the microstructure, see \ref{eq:dt_R}. 
To give a simpler representation of $\textbf{w}_p^\text{nst}$, we first study the normal approach velocity averaged on all $\textbf{r}$, that is,  
\begin{equation*}
    w_{pn}^aP_a(\textbf{x},t,a)
    = \frac{1}{n_p(\textbf{x},t)}
    \int_{\mathbb{R}^3}
    \frac{\textbf{r}}{r} \cdot \textbf{w}^\text{nst}_p
    P_\text{nst}(\textbf{x},\textbf{r},t,a) d\textbf{r}.
\end{equation*}
In this way, $w^\text{a}_{pn}(\textbf{x},t,a)$ is the average relative normal approach velocity between the nearest pair of particles at age $a$. 
The superscript $^a$ indicate that $w_{pn}^a$ is conditioned only on the age $a$. 
It represents the average approach velocity from one particle to its nearest neighbor, measured from the time when the particles became nearest neighbors, $a=0$.
A scheme of what $\frac{\textbf{r}}{r} \cdot \textbf{w}^\text{nst}_p$ is,  is given \ref{fig:normal_vel_picture} (right). 
\begin{figure}[h!]
    \centering
    % \includegraphics[height = 0.4\textwidth]{image/HOMOGENEOUS_NEW/Age_cond/uR_rel.pdf}
    % \includegraphics[height = 0.3\textwidth]{image/HOMOGENEOUS_NEW/Age_cond/r_l_10_PHI_10.pdf}
    \begin{tikzpicture}[ scale = 0.6]
        \node (img) at (-0.7\textwidth,0){\includegraphics[height = 0.4\textwidth]{image/HOMOGENEOUS_NEW/Age_cond/uR_rel.pdf}};
        \filldraw[ gray!50!white](0,0) circle (0.5);
        \filldraw[ gray!50!white](1,3)circle (0.5);
        % \draw[fill=gray,opacity=0.2](5,-0.2)circle (0.5);
        % \draw[fill=gray,opacity=0.2](-3,2)circle (0.5);
        % \draw[fill=gray,opacity=0.2](-5,0.2)circle (0.5);
        \draw(0,0)node[right]{$\textbf{x}_i$};
        \draw[dashed](0,0)--(1,3)node[right]{$\textbf{x}_j$};
        % \draw[very thick,<-,blue](-1,0)--++(0,1)node[right]{$\bm{b}$};
        \draw[very thick,->](1,3)--++(0.9,-1.8)node[above right]{$\textbf{w}^\text{nst}(a)$};
        \draw[very thick,->,red](1,3)--++(-0.5,-1.5)node[left]{$w_{ij,n}(a)$};
        \draw[dashed](1,3)++(0.9,-1.8) -- (1,3)++(-0.5,-1.5);
        \node (ii) at (1,-1){$\textbf{w}_{ij} = \textbf{u}_j - \textbf{u}_i$};
        \node (ii) at (1,-1.6){$w_{ij,n} = \textbf{w}_{ij}\cdot \textbf{r}/|\textbf{r}|$};
        % \draw[very thick,->](0,0)--++(1,0)node[below right]{$\bm{e_x}$};
        % \draw[very thick,->](0,0)--++(0,1)node[left]{$\bm{e_y}$};
        % \draw(3,1)++(199:1)node[above left]{$\beta$} arc(199:159:1);
        % \draw(0,0)++(0:1)node[above right]{$\theta$} arc(0:20:1);
    \end{tikzpicture} 
    \caption{(left) Relative normal approach velocity between two nearest neighbors, averaged conditionally on the age of interaction.  
    The age $a$, as well as the velocity are made dimensionless  with the mean age $\tau_a$ and the length scale $d_p = n_p^{-1/3}$. 
    % The symbols represent the different \textit{Galileo} numbers, the colors the different 
    % ($\pmb\bigcirc$) $Ga=10$; ($\pmb\triangle$) $ Ga = 25$; ($\pmb\square$) $Ga = 50$ ($\pmb\lozenge$) $Ga =100$.
    % The colors represent the different volume fractions, (blue) $\phi =0.01$, (green) $\phi = 0.05$ (organ) $\phi=0.1$ (red) $\phi = 0.2$. 
    % The white symbols correspond to $\lambda = 1$, and black symbols to $\lambda = 10$. 
    (right)
    Scheme of two nearest neighbors with their position $\textbf{x}_i$ and $\textbf{x}_j$, velocities $\textbf{u}_{i}$ and $\textbf{u}_j$, relative velocity $\textbf{w}_{ij}$ and normal relative velocity $w^{ij,n}$. 
    }
    \label{fig:normal_vel_picture}
\end{figure}
The approach velocity $w_{pn}^a(\textbf{x},t,a)$ for all the DNS carried in this work is displayed \ref{fig:normal_vel_picture} (left). 
The x-axis is made dimensionless with the averaged time of interaction, $\tau_p$, and the y-axis is scaled with the velocity scale $d_p /\tau_p$. 
At  early age we observe that $w_{pn}^a<0$.
Then it eventually reaches zero for  $a \approx 0.5\tau_p$.
After this time $w_{pn}^a>0$ and remains constant with respect to $a$. 
Hence, on average, particles approach each other at early ages ($w_{pn}^a<0$), and then they move apart for $a > \tau_p$ with a constant average velocity.

Two important features are identified from \ref{fig:normal_vel_picture} (left).
First, all curves are roughly similar, even if we can see slight differences in magnitude for the different $\phi$. 
Thus, regardless of the flow parameters, $w_{pn}^a(\textbf{x},t,a)$ scale roughly as $d_p /\tau_p$. 
Second,  $w_{pn}^a(\textbf{x},t,a)$ seems to relax for age, $a > \tau_p$, to reaches a constant value. 
% Consequently, it seems that $\tau_p$ is also the relaxation time for the particles' relative normal approach velocity. 
Consequently, we demonstrated that $\tau_p$ and $d_p$ were the correct time and length scale which govern the inter particle scale kinematic, and that $\tau_p$ is also the relaxation time of $w_{pn}^a(\textbf{x},t,a)$. 
% It is clear that all nearest averaged property will be also subject to a relaxation time $\tau_p$, this in fact comes from the structure of the nearest particle averaged probability transport equation (\ref{eq:dt_Pnst}) which makes appear this relaxation time. 
In general, we believe that $w_{pn}^a(\textbf{x},t,a)$ might be useful for the future studies aiming to construct models based on the relative velocity between particles \citep{rao2008introduction}. 



==> microstructure/Velocity.tex <==

In \ref{sec:microstructure} we have investigated the microstructure geometry, 
in \ref{sec:time} we have seen that the timescale governing both, the microstructure evolution and the particles pair relative velocity is $\tau_p$.   
We now give a visual representation of the nearest pair relative velocity in space to better understand how the relative kinematic behave.  
To that end we compute the nearest relative velocity and age, averaged on all ages, that is,
\begin{align*}
    \textbf{w}^\text{r}_pP_r(\textbf{x},\textbf{r},t)
    =\int_0^\infty \textbf{w}^\text{nst}_pP_\text{nst}(\textbf{x},\textbf{r},t,a) da,\\
    a^rP_r(\textbf{x},\textbf{r},t)
    =\int_0^\infty a P_\text{nst}(\textbf{x},\textbf{r},t,a) da.
\end{align*}
The superscript $^\text{r}$ indicate that the quantity $\textbf{w}^\text{r}_p$ and $a^r$ is conditioned on the relative position \textbf{r} only.
As will be demonstrated, having a good estimation of these velocities and ages mean fields allows one to reconstruct the history of the particles' kinematic interactions. 
To be able to visualize
$\textbf{w}^\text{r}_p(\textbf{x},\textbf{r},t)$
and 
$a^r(\textbf{x},\textbf{r},t)$
on 2D plots we consider an axis symmetry along the vertical axis, and average the values of 
$\textbf{w}^\text{r}_p(\textbf{x},\textbf{r},t)$
and $a^r(\textbf{x},\textbf{r},t)$
on the polar coordinate, as it has been done for $P_\text{nst}$ in \ref{sec:microstructure}. 
However, unlike in \ref{sec:microstructure} we do not assume symmetry with respect to the horizontal plane. 

\subsubsection*{Impact of the inertial effects}

The first effect that we study is the impact of the inertial effects on the particles relative kinematic.  
In \ref{fig:Why_Ga_matter} we display the velocity fields $\textbf{w}_p^r$ represented by the arrows that are colored by the mean dimensionless age $a^r$.  
On the left panel, we observe a low inertial case ($Ga = 10$), while on the right panel, we display a highly inertial case ($Ga=100$), both for $\lambda =1$ and $\phi=0.05$.
\begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_10_PHI_5.pdf}
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_100_PHI_5.pdf}
    % \begin{tikzpicture}[scale=0.8]
    %     \filldraw[ gray!50!white](0,0) circle (0.5);
    %     \filldraw[ gray!50!white](1,3)circle (0.5);
    %     \filldraw[ gray!50!white](-0.2,3.5)circle (0.5);
    %     % \draw[fill=gray,opacity=0.2](5,-0.2)circle (0.5);
    %     % \draw[fill=gray,opacity=0.2](-3,2)circle (0.5);
    %     % \draw[fill=gray,opacity=0.2](-5,0.2)circle (0.5);
    %     \draw(0,0)node[right]{$p_1, \; \textbf{x} = 0 $};
    %     \draw[dashed](0,0)--(1,3)node[right]{$p_2, \;\textbf{x}+\textbf{r}$};
    %     \draw[dashed](-0.2,3.5)node[right]{$p_3$};
    % \end{tikzpicture} 
    % \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_10_Ga_10_PHI_5.pdf}
    % \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_10_Ga_100_PHI_5.pdf}
    \caption{
         Quiver plots of the relative averaged velocity field $\textbf{w}^\text{r}(\textbf{x},\textbf{r},t)$ colored by the averaged dimensionless age $a^r(\textbf{x},\textbf{r},t)$ for $\phi = 0.05$ and $\lambda +1$.
         (left) $Ga = 10$ (right) $Ga =100$. }
    \label{fig:Why_Ga_matter}
\end{figure}

The first aspect that we would like to clarify is the non fore-aft symmetry of the velocity fields $\textbf{w}_p^\text{nst}$ with respect to the horizontal plane. 
Indeed, in plots display on \ref{fig:Why_Ga_matter} we remark that the $\textbf{w}_p^\text{nst}$ exhibit a clear asymmetry with respect to the horizontal plane.
This is explained by the non commutativity of the function $h_{ij}$ in the indices $i$ and $j$ in \ref{eq:q_nstij}, as a result $\textbf{w}_p^r(\textbf{x},t,r,\theta) \neq \textbf{w}_p^r(\textbf{x},t,r,-\theta)$. 
Indeed, as it is depicted on \ref{fig:diagram_asym}, in the cases were the neighboring nearest particle is far from the test particle, the chance for this particle to have another nearest neighbor which is closer is high. 
Thus, the nearest neighbor of the nearest neighbor of the test particle, is not necessarily the test particle. 
This induces asymmetry in the nearest neighbor statistics. 
That explains why the plots on \ref{fig:Why_Ga_matter} are not symmetrical when we observe the fields at sufficiently large distance $|\textbf{r}|$. 
Note that this asymmetry would not be present if we had considered classic particle pair average as it is done in \cite{shajahan2023inertial}. 
To summaries, in the situation where we observe $\textbf{w}_p^r$ for large $|\textbf{r}|$ the test particle can be considered as being \textit{isolated}, as its nearest neighbor is at a large distance $|\textbf{r}|$ from the test particle. 
Additionally, the nearest neighboring particle, if located far enough, has 
potentially a nearest neighbor that is closer than the test sphere, as explained on \ref{fig:diagram_asym}. 
Consequently, provided that the nearest neighbor of the test sphere is far enough, we can be sure that on average it approaches a pair of particles or more, that are packed together. 

\begin{figure}[h!]
    \centering
    \hfill
    \begin{tikzpicture}[scale=0.8]
        \filldraw[ gray!10!white](+2.6,3.5)circle (0.5);
        \filldraw[ gray!10!white](-1.5,3.2)circle (0.5);
        \draw[dashed](30:3.16) arc (30:120:3.16);
        \filldraw[ gray!50!white](0,0) circle (0.5);
        \filldraw[ gray!50!white](1,3)circle (0.5);
        \filldraw[ gray!50!white](-0.2,3.5)circle (0.5);
        \draw(0,0)node[right]{$p_1, \; \textbf{x} = 0 $};
        \draw[dashed](0,0)--(1,3)node[right]{$p_2, \;\textbf{x}+\textbf{r}$};
        \draw[dashed](-0.2,3.5)node[right]{$p_3$};
        \node[ultra thick] (title) at (-0.5,1.5) {\textit{Case 1}};
    \end{tikzpicture} 
    \hfill
    \begin{tikzpicture}[rotate=180, xscale=-0.8,yscale=0.8]
        \filldraw[ gray!10!white](+2.6,3.5)circle (0.5);
        \filldraw[ gray!10!white](-1.5,3.2)circle (0.5);
        \draw[dashed](30:3.16) arc (30:120:3.16);
        \filldraw[ gray!50!white](0,0) circle (0.5);
        \filldraw[ gray!50!white](1,3)circle (0.5);
        \filldraw[ gray!50!white](-0.2,3.5)circle (0.5);
        \draw(0,0)node[right]{$p_1, \; \textbf{x} = 0 $};
        \draw[dashed](0,0)--(1,3)node[right]{$p_2, \;\textbf{x}+\textbf{r}$};
        \draw[dashed](-0.2,3.5)node[right]{$p_3$};
        \node[ultra thick] (title) at (-0.5,1.5) {\textit{Case 2}};
    \end{tikzpicture} 
    \hfill
    % \begin{tikzpicture}[scale=0.8]
    %     \filldraw[ gray!10!white](+2.6,3.5)circle (0.5);
    %     \filldraw[ gray!10!white](-1.5,3.2)circle (0.5);
    %     \draw[dashed](-30:3.16) arc (-30:-120:3.16);
    %     \filldraw[ gray!50!white](0,0) circle (0.5);
    %     \filldraw[ gray!50!white](1,-3)circle (0.5);
    %     % \filldraw[ gray!20!white](-1.4,-3.3)circle (0.5);
    %     \filldraw[ gray!50!white](-0.2,-3.5)circle (0.5);
    %     % \draw[fill=gray,opacity=0.2](5,-0.2)circle (0.5);
    %     % \draw[fill=gray,opacity=0.2](-3,2)circle (0.5);
    %     % \draw[fill=gray,opacity=0.2](-5,0.2)circle (0.5);
    %     \draw(0,0)node[right]{$p_1, \; \textbf{x} = 0 $};
    %     \draw[dashed](0,0)--(1,-3)node[right]{$p_2, \;\textbf{x}+\textbf{r}$};
    %     \draw[dashed](-0.2,-3.5)node[right]{$p_3$};
    %     \node[ultra thick] (title) at (-0.5,-1.5) {$Case\; 2$};
    % \end{tikzpicture} 
    \caption{
        Diagram that highlights the asymmetry of the nearest pair statistic when the nearest neighbor is relatively far from the test particle.
        (\textit{Case 1}) Particle $p_1$ with  its nearest neighbor, $p_2$, located at the \underline{top} of it. 
        (\textit{Case 2}) Particle $p_1$ with  its nearest neighbor, $p_2$, located at the \underline{bottom} of it. 
        (\textit{Case 1} and \textit{2})
        In these situations the particle $p_2$ located at $\textbf{x} + \textbf{r}$, is the nearest neighbor of the particle $p_1$ located at $\textbf{x}$. 
        Since $|\textbf{r}|/d$ is assumed to be large, the nearest neighbor of the particle $p_2$ is more likely to be another nearest neighbor than $p_1$ such as the particle $p_3$, which is closer.
        This is due to the rapid decay of $P_\text{nst}$ for large $|\textbf{r}|/d$, see \ref{fig:Pnst_high_Ga}. 
        In these cases the nearest neighbor of $p_1$ is $p_2$, but the contrary is not true, inducing asymmetry in the statistics.  
    }
    \label{fig:diagram_asym}
\end{figure}

Now that this issue has been clarified, we can proceed to interpret the plots in \ref{fig:Why_Ga_matter}.
The beginning of the interactions happen at the early ages, meaning in the dark blue areas in  \ref{fig:Why_Ga_matter}, which are located on the top or bottom of the particle of reference.
The ending of the interactions corresponds to the greater ages, which are represented by the red areas. 
As shown by \ref{fig:Why_Ga_matter} (left), at low \textit{Galileo} number the nearest particle has a tendency to come from the top or bottom and leave through the sides. 
If the nearest particle is at a reasonable distance $|\textbf{r}| < 1.5d$ on the sides of the test particle, we can see that the vertical relative velocity is on average null, but positive in the radial component.
In this area, the age is at its maximum (dark red zone), therefore the interaction come to an end, meaning that the nearest particles get replace by another. 
Note that for the particles at a larger distance of the test particle, say $|\textbf{r}|>2$, have an averaged positive vertical relative velocity. 
As discussed above, in this situation the neighbor on the side is more likely to be closer to another particle. 
Consequently, if the test particle is isolated, with neighboring particles sufficiently far on the side, it will rise on average with a lower velocity than the latter particles.
Thus, particles at contact  seems to get apart because of the non-null radial velocity, and particle at distance seems to get apart because of the non-null vertical velocity.  
Consequently, on average the side-by-side configuration is not stable in this case, which partly explains why the particle distribution doesn't form any layer or such oriented microstructure at these $Ga$.   

% A plausible explanation for this phenomenon is that the leading particle accelerate the trailing particle with its wake on a first stage. 
% Then, the trailing particle arise to the same altitude as the leading particle, but still goes faster than the leading particle due to the acceleration provided by the wake of the latter particle.
% If the particles get in contact then the interaction duration seem to last longer, and the particles might even get trap in a small stagnation zone on the side of the particles.


For high \textit{Galileo} number, see \ref{fig:Why_Ga_matter} (right), the relative averaged velocity is nearly null on the sides and below the test particle. 
It is a statistical representation, meaning that, $\textbf{w}_p^r = 0$, just witnesses of the fact that the particles' relative velocity are not correlated with the relative position in this area. 
Thus, it is hard to say if the area where $\textbf{w}_p^r = 0$ corresponds to actual stagnation zones where both particles are in equilibrium, or if the relative velocity is just not correlated. 
Additionally, the particles at a large distance on the top of the test particle have a downward velocity. 
Meaning that if the test sphere is isolated and approach one or several  particles on the top of it (see \ref{fig:diagram_asym} (\textit{Case 1})), it will eventually catch up the latter particles. 
On the contrary, if the particle is isolated and that the nearest neighbor is at the bottom (see \ref{fig:diagram_asym} (\textit{Case 2})), the velocity is either pointing downward, or it is not correlated with the position, as indicated by the magnitude of $\textbf{w}_p^r$. 
A plausible explanation for this phenomenon is that the reference particle, when being isolated, goes faster than the potentially packed nearest neighbor.
Therefore, the test sphere can either catch up with the nearest particle if it is above, or move further away from it if it is below.
Also, it is interesting to notice that in this case the particles at near contact on the bottom of the test particles results from early interaction, denoted by the dark blue zone. 
It can be interpreted as follows : since 
initial time of interaction is on average low in this zone, it does mean that particles replace an old nearest neighbor that where at near contact of the test particles. 
Thus, in this case the nearest neighbor reaches the test sphere which were rising slowly because of a potentially close neighbor. 

Ultimately, the fields $\textbf{w}^r_p(\textbf{x},\textbf{r}, a)$ provide a quantitative averaged representation of what is known as the \textit{Drafting Kissing Tumbling} \citep{fortes1987nonlinear} mechanism. 
Indeed, in both case particles eventually approach from the verticals (\textit{Drafting}), nearly touch each other (\textit{Kissing}), and leave through the sides (\textit{Tumbling}). 
Statistically, the \textit{Tumbling} part is not present in the high inertial case, which  explains the creation of anisotropic structures or more stable side-by-side configurations. 
For bubble pair interactions \citet{zhang2021three} observed such DKT behavior.
They also reported side-by-side stable configuration of pairs. 
However, at same \textit{Galileo} than  \citet{zhang2021three} ($Ga = 10$) we were not able to identify this pair mechanism. 


To support the deduction made above, we displayed in \ref{fig:unst_ga} the absolute conditioned averaged center of mass velocity of the test sphere, defined as,
\begin{equation*}
    \textbf{u}^\text{r}_p(\textbf{x},\textbf{r},t)  
    =
    \frac{1}{P_r(\textbf{x},\textbf{r},t)}
    \int_0^\infty \textbf{u}^\text{nst}_pP_\text{nst}(\textbf{x},\textbf{r},t,a) da
\end{equation*}
In \ref{fig:unst_ga} (left) we clearly see that the magnitude of the test particle's vertical velocity is higher than the particle phase vertical velocity $\textbf{u}_p$ when the nearest neighbor is at near contact to the test particle, either above or below.
\begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_l_1_Ga_10_PHI_5.pdf}
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_l_1_Ga_100_PHI_5.pdf}
    \caption{
         Quiver plots of the conditioned particle velocity field $\textbf{u}^\text{r}(\textbf{x},\textbf{r},t)$ colored by the averaged dimensionless vertical velocity difference : $(\textbf{u}^\text{r} - \textbf{u}_p )/ \textbf{u}_p$, for $\lambda = 1$ and $\phi = 0.05$. 
         (left) Low \textit{Galileo} number $Ga = 10$.
        (right) High \textit{Galileo} number $Ga = 100$.
         }
    \label{fig:unst_ga}
\end{figure}
When the nearest neighbor is at large distance of the test particle, its average velocity is lower than $\textbf{u}_p$. 
At high inertia however, the test particle velocity is higher when being isolated than with its neighbor at near contact. 
Additionally, we can see that when the particle is on the side at near contact or below, the test sphere's velocity  is lower than the mean. 
In brief in the case of $Ga = 10$ it seems that isolated particles goes slower than close neighbors packed together. 
While at higher \textit{Galileo} number it is the opposite, we observe that isolated particles  goes faster than packed neighbor. 


\subsubsection*{The volume fraction dependency}
As it has been observed in \ref{fig:A} the effect of increasing $\phi$ is that it makes the particle distribution slightly more isotropic for $\phi >0.1$. 
\begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_100_PHI_5.pdf}
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_100_PHI_20.pdf}
    % \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_10_Ga_100_PHI_10.pdf}
    % \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_100_PHI_10.pdf}
    \caption{Quiver plots of the relative averaged velocity field $\textbf{w}^\text{r}(\textbf{x},\textbf{r},t)$ colored by the averaged dimensionless age $a^r(\textbf{x},\textbf{r},t)$, for $Ga = 100$ and $\lambda = 1$. 
    (left) Low \textit{Galileo} number $\phi = 0.05$.
    (right) High \textit{Galileo} number $\phi = 0.2$. }
    \label{fig:Why_Phi_matter}
\end{figure}
In \ref{fig:Why_Phi_matter} we expose two situations with various volume fractions. 
In both graph we observe the same trend, despite the changes in length scales, which are due to the variations in volume fraction. 
Indeed, the stagnation zones with dark red color and the particle resulting from short interactions, dark blue color, are located approximately at the same location. 
We still observe the fore-aft asymmetry with respect to the horizontal plane, as it was discussed above. 
For other $\lambda$ and $Ga$ no particular differences could be observed with varying $\phi$. 
Overall, even if small differences might be present, the change in volume fraction doesn't seem to affect the relative kinematic of interaction between particles. 

\subsubsection*{Influence of the viscosity ratio}

Lastly, we turn our attention to the effect of the viscosity ratio on pair relative kinematic.
The question that we are trying to answer is : why does a smaller viscosity ratio increase the anisotropy of the tensor $\textbf{R}(\textbf{x},t)$ as it is shown in \ref{fig:A}. 
With this objective in mind, we compare two cases at $Ga = 100$ and $\phi =0.05$, where we observe a clear difference between the distributions (see \ref{fig:Pnst_high_Ga}) between $\lambda = 1$ and $\lambda = 10$.
\begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_10_Ga_100_PHI_5.pdf}
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_100_PHI_5.pdf}
    % \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_1_Ga_100_PHI_1.pdf}
    % \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_rel_l_10_Ga_100_PHI_1.pdf}
    \caption{Quiver plots of the relative averaged velocity field $\textbf{w}^\text{r}(\textbf{x},\textbf{r},t)$ colored by the averaged dimensionless age $a^r(\textbf{x},\textbf{r},t)$, for $\phi = 0.05$ and $Ga = 100$. 
    (left) High viscosity ratio $\lambda = 10$.
    (right) Low viscosity ratio, $\lambda = 1$. }
    \label{fig:Why_l_matter}
\end{figure}
As in the previous cases, it is clear that for both cases in \ref{fig:Why_l_matter} the neighboring particle approach on the vertical direction and end up its course on the sides.
As discussed previously, the case on \ref{fig:Why_l_matter} (right) exhibit a clear stagnation zone and asymmetry on a vertical plane. 
On the other hand for $\lambda =10$ the relative velocity on the vicinity of the particle seem to be on average positive in the radial direction. 
In addition, The asymmetry aforementioned is not present in this case. 
As discussed in the previous paragraph, and explained by \ref{fig:diagram_asym}, the presence of the skew asymmetry in the fields $\textbf{w}_p^\text{r}$ about horizontal plane, witnesses for interactions of the isolated particles clusters of particles.
The absence of such asymmetry implies the absence of such interactions, indicating that the particles are more evenly spread. 

As before, it is interesting to investigate the value of the conditional velocity $\textbf{u}^r_p$ to better understand the particles collective interactions. 
Thus, \ref{fig:unst_l} display the fields  $\textbf{u}_p^\text{r}$ for both cases. 
\begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_l_10_Ga_100_PHI_5.pdf}
    \includegraphics[height=0.35\textwidth]{image/HOMOGENEOUS_NEW/Dist/U_l_1_Ga_100_PHI_5.pdf}
    \caption{
         Quiver plots of the conditioned particle velocity field $\textbf{u}^\text{r}(\textbf{x},\textbf{r},t)$ colored by the averaged dimensionless vertical velocity difference : $(\textbf{u}^\text{r} - \textbf{u}_p )/ \textbf{u}_p$, for $\phi = 0.05$ and $Ga = 100$. 
         (left) High viscosity ratio $\lambda = 10$.
         (right) Low viscosity ratio, $\lambda = 1$.
         }
    \label{fig:unst_l}
\end{figure}
On \ref{fig:unst_l} (left) we first notice that $\textbf{u}^\text{r}(\textbf{x},\textbf{r},t)$ behave similarly as the low inertial case display on \ref{fig:unst_ga} (left).
However, for $\lambda = 10$, the isolated particles' velocity is roughly equal to $\textbf{u}_p$. 
If isolated particle rise at the average velocity it is because the isolated particles constitute the majority of the realization since the trace of \textbf{R} is rather high, see \ref{fig:A}.
Therefore, this fact is not particularly relevant as it is just a statistical bias. 
Nevertheless, we can still conclude that for $\lambda = 10$ particles goes faster with a nearest neighbor on top or bottom, while for  $\lambda = 1$ particles goes faster when the nearest neighbor is at large distance. 


\subsubsection*{Discussion}

From \ref{sec:time} we demonstrated that $\textbf{R}(\textbf{x},t)$ follows a transport equation were the tensor $\textbf{W}(\textbf{x},t)$ act as a source term. 
This tensor might be expressed as the symmetric part of $\int_0^\infty \textbf{r} \textbf{w}_p^\text{r} P(\textbf{x},\textbf{r},t) da$. 
Thus, the trends of the $\textbf{w}_p^\text{r}(\textbf{x},\textbf{r},t) $ in terms of the position determine the value of $\textbf{W}(\textbf{x},t)$ and partly determine the final value of $\textbf{R}(\textbf{x},t)$. 
In most of the graphs we observed that the vertical components of $\textbf{w}_p^\text{r}$ where negative when the vertical component of where positive \textbf{r} and vice versa. 
Consequently, $W_{yy}$ must be on average negative, which ultimately contribute to the value of $\textbf{R}(\textbf{x},t)$ and $\textbf{A}(\textbf{x},t)$ through \ref{eq:dt_R} and justify the sign of $A_{xx}$ in \ref{fig:A}. 

% On a different note, we now ask this question : 
% Is the relative velocity fields $\textbf{w}_p^r$ is the cause of the microstructure's shape as it is suggested by \ref{eq:dt_R}. 
% Or does $\textbf{w}_p^r$ is the consequence of microstructure shape, as it could be through looking at the previous graphs ?
% Indeed, on \ref{fig:Why_l_matter} (right), the clear asymmetry with respect to the horizontal plane can be explained as the consequence of cluster  in the flows. 
% Although it is tedious question, we believe that both are true, even if physical parameters also impact $\textbf{w}_p^r$, which makes the microstructure case dependent.  
% Nevertheless, this makes $\textbf{W}(\textbf{x},t)$ potentially a function of $\textbf{R}(\textbf{x},t)$.
% Depending on its relationship with $\textbf{R}(\textbf{x},t)$ this might modify the relaxation time.  
% Thus, a more efficient way to close \textbf{W} by an objective manner would be to study the dynamic of interactions. 
In this work we only provided a kinematics arguments to explain the microstructure shape. 
Of course to fully understand the physics one has to study the dynamic of interaction. 
It is in fact possible in our framework to include such dynamic variable by deriving an equation for \textbf{W} the same way we derived \ref{eq:dt_R} for \textbf{R}.
% In this case it is reasonable to believe that the closure terms for the dynamical equation might be computable theoretically in terms of the physical parameters $Ga$, $\phi$ and $\lambda$. 

==> microstructure/Velocity2.tex <==
\subsection{Carrier phase velocity fields}

In the previous section we explained the microstructure formation with kinematic arguments.
Although we indeed provided an explanation the question that arise now id :
Why does the relative velocity behave as such.
The answer might be obtained based on dynamical arguments as it is done often, in such a way we could explain the relative kinematic.
Nevertheless, the dynamical aspect of the interaction is out of the scope of this study and will be treated in a future work. 

Instead, we propose to study the particles averaged wakes to explain the possible difference in interaction between the iso-viscous and viscous droplets cases. 
Again we make use of the nearest particle averaged statistic to compute the carrier fluid phase velocity conditionally on the presence of a particle at \textbf{x}, it reads,
\begin{equation*}
    \textbf{u}^\text{nst}_f P_{nst}(\textbf{x},\textbf{r},t)= 
    \int \sum_{i}^{N_b} \delta(\textbf{x}-\textbf{x}_i(\FF,t))
    h_{i} 
    \textbf{u}_f^0(\textbf{x}+\textbf{r},t,\FF)
    d\mathscr{P} 
\end{equation*}
where $h_{i} = 1$ if the particle $i$ center of mass is the nearest point to the eularian coordinate \textbf{x}+\textbf{r}. 
This velocity fields can be reconstructed as well with our DNS. 
On \ref{fig:stream} we display the reconstructed velocity field $\textbf{u}^\text{nst}_f$ for (left) the iso-viscous case $\lambda =1$ and (right) the viscous droplets' case $\lambda = 10$, for different value of the volume fraction. 
\begin{figure}[h!]
    \centering
    \includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_1_Ga_100_l_100}
    \includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_1_Ga_100_l_10}
    \includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_5_Ga_5_l_100}
    \includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_5_Ga_5_l_10}
    \includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_20_Ga_100_l_100}
    \includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_20_Ga_100_l_10}
    % \includegraphics{image/HOMOGENEOUS_NEW/Stream/Stream_PHI_5_Ga_100_l_1.pdf}
    \caption{Nearest averaged carrier phase velocity fields. }
    \label{fig:stream}
\end{figure}
This velocity field is evaluated at $\textbf{x}+\textbf{r}$ conditioned on the presence of the nearest particle at $\textbf{x}$. 


\tb{compare with \citet{shajahan2023inertial} for explaination }

==> microstructure/configuration.tex <==







\subsection{Nearest particles arrangements}
\begin{itemize}
    \item Problematic : "How the particles are arranged relative to each other"
    \item Show : "How to compute the Radial and azimuthal probability density function : $P_{nst}(r)$  and $P_{nst}(\theta)$"
    \item  Conclusion on $P_{nst}(\theta)$ : "We observe that the particles pair becomes oriented with increasing $Ga$ and decreasing volume fraction.
    \item  Conclusion on $P_{nst}(r)$ : "We observe that the particles pair becomes randomly arranged for high $Ga$ but in average they are rather spaced from each other" 
\end{itemize}
\tb{Je me demande si cette section est vraiment utile .... car elle n'apport pas d'explication supplementaire a la drag force ni aux fluctuations, c'est peux être mieux de garder ca pour l'article qui traîte des interactions }


\subsubsection{Map at low $Ar$}

\paragraph{low $\phi$}
\begin{figure}
\centering
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_0_1_Ga_10_PHI_0_05}
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_1_0_Ga_10_PHI_0_05}
\end{figure}

\JL{a on la meme echelle de couleur entre les deux graphiques, les cas Ga=5 ne semblent pas converger ? a virer ...}

Pas de position preferentiel dans ce cas

\paragraph{high $\phi$}
\begin{figure}
\centering
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_0_1_Ga_10_PHI_0_15}
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_1_0_Ga_10_PHI_0_15}
\end{figure}

Idem pas de position preferentiel a discuter a la lumiere de la litterature (qui tends a dire le contraire ?). En regime de Stokes pas d'effet significatif du rapport de viscosité sur les pertubations. 







\subsubsection{Map at high $Ar$}

\paragraph{low $\phi$}
\begin{figure}
\centering
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_0_1_Ga_75_PHI_0_05}
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_1_0_Ga_75_PHI_0_05}
\end{figure}

enorme effet du rapport de viscosité (donc a priori du sillage).
\JL{il manque des cas a Ga=100 ?}


\paragraph{high $\phi$}
\begin{figure}
\centering
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_0_1_Ga_75_PHI_0_15}
\includegraphics[width=4cm]{image/HOMOGENEOUS/fDrop/Pnst_mu_r_1_0_Ga_75_PHI_0_15}
\end{figure}

\subsubsection{...}


\begin{figure}
    \centering
    \begin{tikzpicture}
        \node at (0,0){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_theta_mu_r_1_0_Ga_10.pdf} };
        \node at (0.4\textwidth,0){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_theta_mu_r_0_1_Ga_10.pdf} };
        \node at (0,-0.3\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_theta_mu_r_1_0_Ga_75.pdf} };
        \node at (0.4\textwidth,-0.3\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_theta_mu_r_0_1_Ga_100.pdf} };
        % \node at (0,-0.6\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_theta_mu_r_1_0_Ga_100.pdf} };
        % \node at (0.4\textwidth,-0.6\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_theta_mu_r_0_1_Ga_100.pdf} };
    \end{tikzpicture}
    \caption{Probability density function of the nearest particles : $P_{nst}(\theta)$ for different $Ga$ and $\lambda$. 
    Increasing $Ga$ from top to bottom, (left) $\lambda = 1$ (right) $\lambda = 10$. 
    The symbols correspond to different volume fraction ($\bullet$) $\phi = 1\%$, ($\blacktriangle$) $\phi = 5\%$, ($\blacksquare$) $\phi = 10\%$, ($\blacklozenge$) $\phi = 15\%$ and ($\blacktriangleright$) $\phi = 20\%$.
    (dashed lines) empirical formulas }
    \label{fig:P_nst_theta}
\end{figure}
By using polar coordinate such that $d \textbf{r} = r^2 \sin \phi dr d\phi d\theta$ we can further reduce the PDF to the only consideration of the angular dependency $\theta$ or the distance dependency $r$. 
These reduced p.d.f can be computed as follow, 
\begin{align*}
    P_{nst}(r) 
    &= \int_{-\pi/2}^{\pi/2}\int_{0}^{2\theta} P_{nst}(\textbf{x},\textbf{r},t) \sin \theta  d\phi d\theta\\
    P_{nst}(\theta)
    &= \int_{0}^{\infty}\int_{0}^{2\theta} P_{nst}(\textbf{x},\textbf{r},t) r^2  dr d\phi
\end{align*}
\tb{Check if those formulas are true}
Then $P_{nst}(\theta)$ is the probability that the nearest neighbor of a test particle is inclined at an angle $\theta$ relative to the flow direction. 
We observe that the particles pair becomes oriented with increasing $Ga$ and decreasing volume fraction

On \ref{fig:P_nst_theta} we observe that the particles pair becomes oriented with increasing $Ga$ and decreasing volume fraction.
Indeed, we observe a clear peak of $P_{nst}(\theta)$ at $\theta = \frac{\pi}{2}$. 
It seems that this tendency was also reported for spherical bubble in air-water system \citet{bunner2003effect}. 
Additionally, from \ref{fig:P_nst_theta} we can say that the viscosity ratio $\lambda$ seem to prevent the alignment/clustering of particles denoted by the slightly low peak for $\lambda =10$. 
\tb{Compart the Orientation with bubbly and solid flows \citet{roghair2011drag}}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node at (0,0){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_r_mu_r_1_0_PHI_1.pdf} };
        \node at (0.4\textwidth,0){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_r_mu_r_0_1_PHI_1.pdf} };
        \node at (0,-0.3\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_r_mu_r_1_0_PHI_10.pdf} };
        \node at (0.4\textwidth,-0.3\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_r_mu_r_0_1_PHI_10.pdf} };
        \node at (0,-0.6\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_r_mu_r_1_0_PHI_20.pdf} };
        \node at (0.4\textwidth,-0.6\textwidth){ \includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/Pnst_r_mu_r_0_1_PHI_20.pdf} };
    \end{tikzpicture}
    \caption{Radial probability density function : $P_{nst}(r)$ for different $\phi$ and $\lambda$. 
    Increasing $\phi$ from top to bottom, (left) $\lambda = 1$ (right) $\lambda = 10$. 
    The symbols correspond to different Galileo number ($\bullet$) $Ga = 10$, ($\blacktriangle$) $Ga = 25$, ($\blacksquare$) $Ga = 50$, ($\blacklozenge$) $Ga = 75$ and ($\blacktriangleright$) $Ga = 100$.
    (dashed lines) Theoretical formula \ref{eq:P_nst_r}}
    \label{fig:P_nst_r}
\end{figure}
Note that for solid spherical particle in the dilute regime a theoretical formula for $P_{nst}(r)$ can be found assuming completely random distribution and no interactions nor overlap between particles \citep{zhang2021ensemble}, it reads, 
\begin{equation*}
    P_\text{nst}^\text{th}(r) = n_p e^{-4 \pi n_p (r^3 - d^3)/3}.
    \label{eq:P_nst_r}
\end{equation*}
It is evident that all the distribution presented \ref{fig:P_nst_r} have a peak at $r > 1$ where the theoretical formula  predict a peak at $r=1$. 
This is obviously due to the fact that we are in presence of particles interaction which tends to repulse the particles from each others and therefore to shift the distribution to the left. 
What is more interesting is that for $\lambda = 1$ at low volume fraction and high \textit{Galileo} we are able to recover approximately the random particle distribution $P_\text{nst}^\text{th}$ with our numerical results. 
Whereas for $\lambda = 10$ the particle are relatively maintained far from  each other as depicted \ref{fig:P_nst_r}(right). 
We can stipulate that for high viscosity ratio the particles have a tendency to generate more particle fluid mediated interaction as demonstrated by the flow lines \ref{fig:Stream}.


\subsection{Nearest-particle average fluid velocity}
Objectives : 
\begin{itemize}
    \item Problematic "How to analyse the flow around a particle in average"
    \item First : present the averaged the nearest particles' statistics method. And how to compute the nearest averaged velocity fields $\nstavg{\textbf{u}}$.
    \item Present the flowlines and show that for $\phi = 5 \rightarrow 20\%$ we observe that a vertical symmetry arise.
    \item Explain how this field it is related to the velocity fluctuation with \ref{eq:def_uu}
    \item Conclude that these velocity fields represent the PWFs since it represent the mean wakes \citep{du2022analysis}.  
    \item Additionally, some comment can be made regarding the shape of the particle thanks to the contour lines. 
    \item Approach these flow fields by analytical solution of potential flow to obtain an analytical solution for teh reyolds stress. 
\end{itemize}

Presently, we wish to investigate the  averaged flow structure around a fluid particle.
To obtain such a field we make use of the nearest particle statistics recently introduced by \citet{zhang2021stress}. 
We introduce $\nstavg{\textbf{u}}(\textbf{x},\textbf{r})$ as the velocity fields at \textbf{x} knowing there is a particles center of mass located at \textbf{r}.
Additionally, this particle is the nearest particle among all to the point \textbf{x}.  
Formally, this conditional average can be written as, 
\begin{equation}
    \nstavg{\textbf{u}}(\textbf{x},\textbf{r})=\frac{1}{P_{nst}(\textbf{x},\textbf{r})} 
    \int \textbf{u}(\textbf{x},\CC,t) 
    \sum_{\alpha}\delta(\textbf{x}+\textbf{r}-\textbf{x}^\alpha(\CC,t)) h_{\alpha}(\CC,\textbf{x},t) d\mathscr{P} 
    \label{eq:q_nst_avg}
\end{equation}
where $P_{nst}(\textbf{x},\textbf{r})$ is defined as,  
\begin{equation}
    P_{nst}(\textbf{x},\textbf{r})= 
    \int
    \sum_{\alpha}\delta(\textbf{x}+\textbf{r}-\textbf{x}^\alpha(\CC,t)) 
    h_\alpha(\CC,\textbf{x},t) d\mathscr{P}. 
    \label{eq:P_nsti}
\end{equation}
which is the probability of finding a particle center of mass at a distance \textbf{r} from the point \textbf{x} knowing that this particle is the nearest neighbor to the points \textbf{x}. 
The function $h_\alpha$ is defined such that, $h_\alpha = 1/N^p$ if $\alpha$ is the nearest particle to \textbf{x} and $0$ if not, where $N^p$ is the total number of nearest neighbor.
Indeed, the point \textbf{x} at mid-distance from two particles posses two nearest neighbors by definition, thus $N(\textbf{x},\CC,t) = 2$ in this case. 

\tb{Include the numerical computaiton of $\nstavg{\textbf{u}}$.  }

\ref{fig:Stream} shows the streamline of the field $\nstavg{\textbf{u}}(\textbf{x},\textbf{r})$ for three volume fractions. 
We clearly observe the induced wake of the particles centered at the origin. 

\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
        \node (img) at (0,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_20_Ga_10_l_1.pdf}};
        \node (img) at (0.3\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_20_Ga_50_l_1.pdf}};
        \node (img) at (0.6\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_20_Ga_100_l_1.pdf}};
        \node (img) at (0,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_20_Ga_10_l_10.pdf}};
        \node (img) at (0.3\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_20_Ga_50_l_10.pdf}};
        \node (img) at (0.6\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_20_Ga_100_l_10.pdf}};
        \node (img) at (0,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_5_Ga_10_l_1.pdf}};
        \node (img) at (0.3\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_5_Ga_50_l_1.pdf}};
        \node (img) at (0.6\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_5_Ga_100_l_1.pdf}};
        \node (img) at (0,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_5_Ga_10_l_10.pdf}};
        \node (img) at (0.3\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_5_Ga_50_l_10.pdf}};
        \node (img) at (0.6\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/Stream_PHI_5_Ga_100_l_10.pdf}};
    \end{tikzpicture}
    \caption{Nearest particle averaged velocity $\nstavg{\textbf{u}}(\textbf{r})$ for  $\phi = 5\%$ and $20\%$.
    Green lines : contour plots of the nearest averaged indicator function $\nstavg{\chi_d}(\textbf{r})$ (it represent the mean shape of the particles)}
    \label{fig:Stream}
\end{figure}
% \begin{figure}[h!]
%     \centering
%     \begin{tikzpicture}
%         \node (img) at (0,0)  {\includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_10_l_1.pdf}};
%         \node (img) at (0.3\textwidth,0)  {\includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_50_l_1.pdf}};
%         \node (img) at (0.6\textwidth,0)  {\includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_100_l_1.pdf}};
%         \node (img) at (0,0.4\textwidth)  {\includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_10_l_10.pdf}};
%         \node (img) at (0.3\textwidth,0.4\textwidth)  {\includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_50_l_10.pdf}};
%         \node (img) at (0.6\textwidth,0.4\textwidth)  {\includegraphics[height=0.4\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_100_l_10.pdf}};
%     \end{tikzpicture}
%     \caption{Nearest particle averaged pressure $\nstavg{p}(\textbf{r})$ normalized by the Laplace pressure $4 \gamma /d$ for  $\phi = 5\%$ and $20\%$}
%     \label{fig:Stream}
% \end{figure}
\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
        \node (img) at (0,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_10_l_1.pdf}};
        \node (img) at (0.3\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_50_l_1.pdf}};
        \node (img) at (0.6\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_100_l_1.pdf}};
        \node (img) at (0,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_10_l_10.pdf}};
        \node (img) at (0.3\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_50_l_10.pdf}};
        \node (img) at (0.6\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_20_Ga_100_l_10.pdf}};
        \node (img) at (0,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_10_l_1.pdf}};
        \node (img) at (0.3\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_50_l_1.pdf}};
        \node (img) at (0.6\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_100_l_1.pdf}};
        % \node (img) at (0,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_10_l_10.pdf}};
        \node (img) at (0.3\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_50_l_10.pdf}};
        \node (img) at (0.6\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/Stream/P_PHI_5_Ga_100_l_10.pdf}};
    \end{tikzpicture}
    \caption{Nearest particle averaged pressure $\nstavg{p}(\textbf{r})$ normalized by the Laplace pressure $4 \gamma /d$ for  $\phi = 5\%$ and $20\%$}  
    \label{fig:Stream}
\end{figure}
It is evident from these plots that the induced wake is the averaged wake resulting from the averaged translation of the particles. 
And this averaged wake has a tendency to be asymmetrical for low volume fraction and symmetrical for higher ones. 
Additionally, form basic mathematical consideration on the average operators we can demonstrate that :
\begin{multline*}
    \avg{\chi_k \textbf{u}'_k\textbf{u}'_k}(\textbf{x},t)
    + \phi_k \textbf{u}_k\textbf{u}_k
    = \\
    \underbrace{\int (\nstavg{\chi_k \textbf{u}^0_k}  \nstavg{\chi_k \textbf{u}^0_k} / (\nstavg{\chi_k})  P_{nst}(\textbf{x},t,\textbf{r}) d\textbf{r} }_\text{PWFs}
    +\underbrace{\int \nstavg{\chi_k \textbf{v}_k^0\textbf{v}_k^0}  P_{nst}(\textbf{x},t,\textbf{r}) d\textbf{r}}_\text{WIA}
    \label{eq:def_uu}
\end{multline*}
where, $\textbf{v}_k^0  = \textbf{u}_k^0 - \nstavg{\chi_k \textbf{u}^0_k} / \nstavg{\chi_k}$ is the fluctuation of the local velocity relative to the nearest averaged value. 
Consequently, we can decompose the ensemble averaged fluid velocity fluctuations with a first term representing the variance of $\nstavg{\textbf{u}}$ around the mean $\textbf{u}_k$, and a second term representing the variance of $\textbf{u}^0_k$ around the mean  $\nstavg{\textbf{u}}$. 

There are two phenomena causing velocity fluctuations in the liquid:
the agitation resulting from wakes and their collective interactions [wake-induced agitation (WIA)], and the non-turbulent fluctuations resulting from averaged wakes and potential flows around bubbles [potential flow and averaged wake fluctuations (PWFs)].
As a matter of fact in the phase space of $\nstavg{\textbf{u}}(\textbf{r})$ the bubble is fixed at the origin thus we recover the velocity fields representing what is called the PWFs. 
In their study \citet{du2022analysis} carry out transient simulation with fixed particles to recover the PWFs components here we show that a single simulation permit us to recover WIA and PWFs by the mean of the nearest particles' statistics. 

\tb{make the link with drag force/drag coef  \citet{dandy1989buoyancy}}
\tb{make the link with velocity fluctuation \citet{almeras2021statistics}}





\subsection{Nearest averaged particle center of mass velocity}
\subsubsection{Nearest averaged particle center of mass velocity in the dispersed phase reference frame}
\begin{equation}
    \nstavg{\textbf{u}^i}=\frac{1}{P_{nst}(\textbf{x},\textbf{r},t)} 
    \int \sum_{i}\delta(\textbf{x}-\textbf{x}^i(\CC,t))
    \sum_{j\neq i}\delta(\textbf{x}+\textbf{r}-\textbf{x}^j(\CC,t)) 
    % \delta(t+a-t_c^{ij}(\CC,t)) 
    h_{ij}(\CC,t) 
    \textbf{u}^i(\CC,t)
    d\mathscr{P} 
    - \textbf{u}_p
\end{equation}
\subsubsection{Nearest averaged particle center of mass relative velocity}
\begin{equation}
    \nstavg{\textbf{w}}=\frac{1}{P_{nst}(\textbf{x},\textbf{r},t)} 
    \int \sum_{i}\delta(\textbf{x}-\textbf{x}^i(\CC,t))
    \sum_{j\neq i}\delta(\textbf{x}+\textbf{r}-\textbf{x}^j(\CC,t)) 
    % \delta(t+a-t_c^{ij}(\CC,t)) 
    h_{ij}(\CC,t) 
    (\textbf{u}^i(\CC,t) - \textbf{u}^j(\CC,t))
    d\mathscr{P} 
\end{equation}


\begin{figure}[h!]
    \centering
    \begin{tikzpicture}
        \node (img) at (0,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_1_Ga_10_PHI_20.pdf}};
        \node (img) at (0.3\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_1_Ga_50_PHI_20.pdf}};
        \node (img) at (0.6\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_1_Ga_100_PHI_20.pdf}};
        \node (img) at (0,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_10_Ga_10_PHI_20.pdf}};
        \node (img) at (0.3\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_10_Ga_50_PHI_20.pdf}};
        \node (img) at (0.6\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_10_Ga_100_PHI_20.pdf}};
        \node (img) at (0,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_1_Ga_10_PHI_5.pdf}};
        \node (img) at (0.3\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_1_Ga_50_PHI_5.pdf}};
        \node (img) at (0.6\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_1_Ga_75_PHI_5.pdf}};
        \node (img) at (0,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_10_Ga_10_PHI_5.pdf}};
        \node (img) at (0.3\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_10_Ga_50_PHI_5.pdf}};
        \node (img) at (0.6\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_l_10_Ga_75_PHI_5.pdf}};
    \end{tikzpicture}
    \caption{Nearest particle averaged pressure velocity $\nstavg{\textbf{u}^i}(\textbf{r}) - \textbf{u}_p$ }  
    \ref{fig:u_nst}
\end{figure}
% \begin{figure}[h!]
%     \centering
%     \begin{tikzpicture}
%         \node (img) at (0,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_1_Ga_10_PHI_20.pdf}};
%         \node (img) at (0.3\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_1_Ga_50_PHI_20.pdf}};
%         \node (img) at (0.6\textwidth,0)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_1_Ga_100_PHI_20.pdf}};
%         \node (img) at (0,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_10_Ga_10_PHI_20.pdf}};
%         \node (img) at (0.3\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_10_Ga_50_PHI_20.pdf}};
%         \node (img) at (0.6\textwidth,-0.3\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_10_Ga_100_PHI_20.pdf}};
%         \node (img) at (0,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_1_Ga_10_PHI_5.pdf}};
%         \node (img) at (0.3\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_1_Ga_50_PHI_5.pdf}};
%         \node (img) at (0.6\textwidth,-0.6\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_1_Ga_75_PHI_5.pdf}};
%         \node (img) at (0,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_10_Ga_10_PHI_5.pdf}};
%         \node (img) at (0.3\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_10_Ga_50_PHI_5.pdf}};
%         \node (img) at (0.6\textwidth,-0.9\textwidth)  {\includegraphics[height=0.3\textwidth]{image/HOMOGENEOUS/fDrop/U_rel_l_10_Ga_75_PHI_5.pdf}};
%     \end{tikzpicture}
%     \caption{Nearest particle averaged pressure velocity $\nstavg{\textbf{w}}(\textbf{r})$ }  
%     \ref{fig:w_nst}
% \end{figure}

